Why Aren't Regular Expressions a Lingua Franca? An Empirical Study on the Re-use and Portability of Regular Expressions

This paper explores the extent to which regular expressions (regexes) are portable across programming languages. Many languages offer similar regex syntaxes, and it would be natural to assume that regexes can be ported across language boundaries. But can regexes be copy/pasted across language boundaries while retaining their semantic and performance characteristics? In our survey of 158 professional software developers, most indicated that they re-use regexes across language boundaries and about half reported that they believe regexes are a universal language. We experimentally evaluated the riskiness of this practice using a novel regex corpus -- 537,806 regexes from 193,524 projects written in JavaScript, Java, PHP, Python, Ruby, Go, Perl, and Rust. Using our polyglot regex corpus, we explored the hitherto-unstudied regex portability problems: logic errors due to semantic differences, and security vulnerabilities due to performance differences. We report that developers' belief in a regex lingua franca is understandable but unfounded. Though most regexes compile across language boundaries, 15% exhibit semantic differences across languages and 10% exhibit performance differences across languages. We explained these differences using regex documentation, and further illuminate our findings by investigating regex engine implementations. Along the way we found bugs in the regex engines of JavaScript-V8, Python, Ruby, and Rust, and potential semantic and performance regex bugs in thousands of modules.

==> related-work-notes.tex <==
% Regexes

% Historical perspective on reuse

% Code reuse
  % Across code, clones or not

  % Code clones
  % From SO
% Problems occuring from reuse

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work} \label{section:RelatedWork}

\FS{This is the new related work section. I kept the old one commented out below for comparison.}

\mysubsection{Empirical studies of regexes.}
The empirical study of regex use is a recent endeavor.
Several lines of research have resulted.
Chapman and Stolee assessed the use of different regex features in Python~\cite{Chapman2016RegexUsageInPythonApps}.
Chapman \etal assessed the understandability of functionally-equivalent regexes and determined community preferences based on the Chapman and Stolee's Python corpus~\cite{Chapman2017RegexComprehension}.
Wang and Stolee have reported that regexes appear to be relatively poorly tested in Java applications~\cite{Wang2018RegexTestCoverage}.
This is in spite of the existence of specific tools for testing and finding semantic problems in regexes, \eg \cite{Larson2016EvilTestStrings,Larson2018AutomaticCheckingOfRegexes,Veanes2010Rex,Arcaini2017MutRex,Larson2016EvilTestStrings,Shen2018ReScueGeneticRegexChecker,Moller2010Brics}.
% We used some of these in our experiments.
Similarly, Staicu \etal \cite{Staicu2018REDOS} proposed a specific tool to identify performance problems (SL regexes), and Davis \etal \cite{Davis2018EcosystemREDOS} reported that they appear in 1-3\% of the modules in the \npm and \pypi registries.

% how we're different
Our polyglot regex corpus will permit the generalization of some of these results to other programming languages.


% Reuse from other code
\mysubsection{Software reuse from other code.}
Software reuse is a prevalent practice in software engineering \cite{Frakes2005,scacchi07fse}.
Software developers opportunistically copy-paste code from their own or others' repositories \cite{sim98}, introducing what are commonly known as \emph{code clones} \cite{roy09sci,gharehyazie18}.
Multiple studies estimate that more than 50\% of the code in Github is duplicated \cite{mockus07,lopes17emse}, and similar ratios have been observed for code in mobile app markets \cite{ruiz12}.

% pros
Some researchers studied positive use cases for code clones, \eg \cite{ossher11}, such as extensions of popular third-party libraries, and found limited differences between cloned and non-cloned code for desirable qualities, such as comprehensibility \cite{saini18} or defect-proneness \cite{rahman12,sajnani14a}.
% cons
In contrast, other studies have looked into many negative effects that could come from cloning code \cite{juergens09}, such as the error-proneness of their maintenance \cite{fowler99}, since they are changed more than other code \cite{lozano07}, but consistently only about half of the time \cite{krinke07}.
% tools to detect them
As a result, a wide variety of techniques have been proposed to detect code clones, \eg \cite{saini18fse,roy09sci,rattan13}.

% how we're different
To the extent of our knowledge, this paper presents the first study of regex reuse and the problems that can arise from it.

% reuse from SO
\mysubsection{Software reuse from Internet forums.}
Software reuse has also been studied from Internet forums --- mostly from Stackoverflow.
Multiple studies found evidence of code flow from Stackoverflow to software repositories \cite{yang17msr,Abdelkareem2017SOCodeReuseInAndroid}, and found that code often flows to multiple programming languages \cite{Allamanis2013SOQuestions}, sometimes without respecting license terms \cite{an17} or authorship attribution \cite{baltes18emse}, and studying the interplay of developer contributions to both resources \cite{vasilescu13}.

% benefits
Given the prevalence of code snippets in Stackoverflow, multiple tools have been proposed to help developer reuse them, \eg to automatically generate comments \cite{wong13}, or to augment the IDE \cite{ponzanelli13,ponzanelli14}.
% problems
However, some problems have been identified with reusing code snippets from Stackoverflow, such as their sometimes (limited) quality \cite{nasehi12} and usability \cite{yang16}.
Furthermore, other studies have identified particular threats with code reuse from Stackoverflow, such as introducing misused APIs \cite{zhang18icse}, security vulnerabilities \cite{fischer17}, or code that is hard to understand \cite{treude17icsme}.

% how we're different
We found in this paper that Internet forums are also a popular source of regex reuse among developers, and we observed risk for similar kinds of problems, \eg introducing \REDOS vulnerabilities.







% Bibliography


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Papers that I want to read their related work section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Papers that I read their related work section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

gharehyazie18
  cross-project code clones in github 
  https://link.springer.com/content/pdf/10.1007%2Fs10664-018-9648-z.pdf

  lopes17
    DéjàVu: a map of code duplicates on GitHub
    https://dl.acm.org/ft_gateway.cfm?id=3133908&type=pdf

saini18esem
  https://link.springer.com/content/pdf/10.1007/s10664-017-9572-7.pdf

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Papers in categories
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Measure the extent of code duplication
  Mockus2007CodeReuse
    Large-scale code reuse in open source software
    http://web.eecs.utk.edu/~audris/papers/ossreuse.pdf
    - A study showed that often more than 50\% of the source code files are reused in more than one open-source projects
    - performed an analysis of popular open source projects, including several versions of Unix and several popular packages; 38K projects and 5M files. The concept of duplication there was simply based on file names. Approximately half of the file names were used in more than one project.

  lopes17
    DéjàVu: a map of code duplicates on GitHub
    https://dl.acm.org/ft_gateway.cfm?id=3133908&type=pdf
    More than 50\% of code is duplicated in Github
    It is an index of duplication for the entire GitHub repository for four popular languages, Java, C++, Python and JavaScript. 

  ruiz12
    Understanding reuse in the android market
    https://ieeexplore.ieee.org/iel5/6230782/6240470/06240477.pdf
    on average 61\% of the total number of classes in each category occurs in two or more mobile apps. 

% Benefits of code duplication

  saini18
    Cloned and non-cloned Java methods: a comparative study
    https://link.springer.com/content/pdf/10.1007/s10664-017-9572-7.pdf
    Found that cloned methods are smaller, perform fundamentally different functions, but no statistically significant difference in terms of usability of comments or comprehensibility.

 This finding is also supported by Sajnani et al. (2014a), where they conducted an
empirical study comparing the presence of bug patterns in cloned and non-cloned code on
36 open source Java projects. Surprisingly, they found that the defect density of cloned code
is less than 2 times the defect density of the non-cloned code.

Sajnani H, Saini V, Lopes CV (2014a) A comparative study of bug patterns in Java cloned and noncloned code. In: IEEE 14th international working conference on source code analysis and manipulation
(SCAM), 2014. IEEE, pp 21–30


% Problems with code duplication
  Juergens09
    Do code clones matter? 
    https://ieeexplore.ieee.org/abstract/document/5070547
  
  Lozano A, Wermelinger M, Nuseibeh B (2007) Evaluating the harmfulness of cloning: a change based experiment. In: Mining software repositories, pp 18–22
  
  Krinke J (2007) A study of consistent and inconsistent changes to code clones. In: Working conference on reverse engineering, pp 170–178

  Bettenburg12
    inconsistent changes to clones 
    https://www.sciencedirect.com/science/article/pii/S0167642310002091

  It has been argued that code cloning adversely impacts software by forcing the tracking of all pieces of code when a certain fault is known to exist, or a new behavior is required, a task that can easily be error prone.

% Code clone detection techniques
  - saini18fse 
    https://arxiv.org/pdf/1806.05837.pdf
    One of the latest approaches to code cloning that uses deep learning to find clones in the twilight zone
  
  roy09sci
    Comparison and evaluation of code clone detection techniques and tools: a qualitative approach. 
    https://www.sciencedirect.com/science/article/pii/S0167642309000367
  
  rattan13
    Clone detection review 
    https://www.sciencedirect.com/science/article/pii/S0950584913000323

%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% reuse silver bullet

cathedral and bazaar 
  http://www.catb.org/esr/writings/cathedral-bazaar/cathedral-bazaar/cathedral-bazaar.ps

scacchi07fse 
  http://www.idi.ntnu.no/grupper/su/courses/tdt10/curricula2010/P4-2-Scacchi07.pdf


% code clones / reuse
- saini18fse 
  https://arxiv.org/pdf/1806.05837.pdf
  One of the latest approaches to code cloning that uses deep learning to find clones in the twilight zone

  These are well-known approches to source code clone
  detection; details of these techniques can be be found in [42]


cross-project code clones in github https://link.springer.com/content/pdf/10.1007%2Fs10664-018-9648-z.pdf
  Coding from scratch is expensive, in terms of both time and effort. So, programmers
  opportunistically reuse code and do so frequently (Juergens et al. 2009).
  Often, programming of well-defined problems amounts to simple look-up (Sim et al.
  1998), first in one’s own, and then in others’ code repositories, followed by judicious copying and pasting. The bigger the corpus of code available, the more likely it is that one will find what one is looking for Gabel and Su (2010).
  The advent of software forges like GitHub and Google Code, and Q&A sites like Stack
  Overflow, has significantly enhanced this kind of opportunistic code reuse (Bajracharya
  et al. 2006; Reiss 2009; Thummalapenta and Xie 2007; Ponzanelli et al. 2014); one can
  readily forage online for code and ideas, and often reuse existing code. In fact, per Open
  Source ideology, developers not only look for the opportunity to reuse code but also
  advertise their own high-quality code for others to reuse in paste-bin like web applications such as GitHub Gist (https://gist.github.com/), Pastebin (http://pastebin.com/), and
  Codeshare (https://codeshare.io/).
  Social coding ecosystems like GitHub present a fundamental shift in reuse opportunities.
  With millions of available OSS projects hosted in GitHub, among which thousands of developers freely migrate, GitHub provides an excellent opportunity for collaboration and code
  reuse (Scacchi 2010; Dabbish et al. 2012); in fact, GitHub actively facilitates the process
  by providing features like advanced code search and GitHub gist. The reused code varies in
  size, ranging from few lines of code to methods, and even larger—one can copy and reuse
  an entire project or a set of files and make smaller modifications to cater to local needs (Ray
  and Kim 2012).1 Thus, ecosystem level code sharing and reuse may be different from within
  project code reuse—one would expect limited methods and file copies in a within project
  setting, resulting in new kinds of software development practices. In this paper we focus on
  studying such ecosystem level code sharing and reuse across multiple GitHub projects.
  An established way to study code reuse is by analyzing code clones (Ray et al. 2014;
  Nguyen et al. 2013). A “clone” is a snippet of code somewhere that is surprisingly similar
  to code elsewhere, and can arise from copy-pasting practices (Kim et al. 2004), automatic
  program generators (Goues et al. 2012; Meng et al. 2011, 2013), or even emerge independently, due to the predictable syntax of underlying programming languages and API usage
  (Al-Ekram et al. 2005). Clones have been studied extensively in the literature, primarily
  within single-project boundaries (Kim et al. 2005; Kamiya et al. 2002),
  as at the time, in the absence of the Web 2.0 and environment-unifying source forges,
  searching and reusing code from other projects would have been challenging. In the past
  5-8 years, GitHub has emerged as a universal platform for maintaining repositories, with
  minimal boundaries between projects. It and other source forges have increased code sharing and reuse, and by virtue of their historical maintenance features, are now enabling us to
  study code cloning across projects

  ( see related work section)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SO and Github


% Flow exists
Yang18msr 
  https://arxiv.org/pdf/1705.01198.pdf
   Near-duplication shows 405k
  distinct blocks (1.1%) in GH being similar to SO and 35k (2%)
  SO distinct blocks having near duplicates in GH. Although the
  percentages are not very large, the numbers are in thousands.
  Upon careful qualitative analysis, we observed that the vast
  majority of these duplicates are very small, typically 2 lines
  of code and just a few tokens. Moreover, they tend to be nondescriptive, meaning that they are too generic to trace. Because
  they are generic and small, likely they didn’t flow from SO to
  GH or vice versa. We then focused out attention to the fewer
  blocks that are not so small. For these, we found evidence that
  there is, indeed, flow from SO to GH, in some cases that flow
  being explicitly stated in comments. While there is a lot less
  of these, their number is still in the thousands.

L. An, O. Mlouki, F. Khomh, and G. Antoniol, “Stack overflow: a
code laundering platform?” in Proceedings of the 24th International
Conference on Software Analysis, Evolution, and Reengineering, ser.
SANER’17, 2017.
  conducted a case study with 399 Android
  apps, to investigate whether developers respect license terms
  when reusing code from SO posts (and the other way around).
  They found 232 code snippets in 62 Android apps that were
  potentially reused from SO, and 1,226 SO posts containing
  code examples that are clones of code released in 68 Android
  apps, suggesting that developers may have copied the code of
  these apps to answer SO questions

B. Vasilescu, V. Filkov, and A. Serebrenik, “Stackoverflow and github:
Associations between software development and crowdsourced knowledge,” in 2013 International Conference on Social Computing, Sept
2013, pp. 188–195.
  social coding dynamics



% Quality of SO code
S. M. Nasehi, J. Sillito, F. Maurer, and C. Burns, “What makes a good
code example?: A study of programming q&a in stackoverflow,” in
28th IEEE International Conference on Software Maintenance, ICSM
2012, Trento, Italy, September 23-28, 2012, 2012, pp. 25–34. [Online].
Available: http://dx.doi.org/10.1109/ICSM.2012.6405249
  Quality of SO code


D. Yang, A. Hussain, and C. V. Lopes, “From query to usable code:
An analysis of stack overflow code snippets,” in Proceedings of the
13th International Conference on Mining Software Repositories, ser.
MSR ’16. New York, NY, USA: ACM, 2016, pp. 391–402. [Online].
Available: http://doi.acm.org/10.1145/2901739.2901767
  provide a usability study of code snippets of four popular programming languages.



% techniques to find them

E. Wong, J. Yang, and L. Tan, “Autocomment: Mining question and
answer sites for automatic comment generation,” in Proceedings of the
2013 IEEE/ACM 28th International Conference on Automated Software
Engineering (ASE). ACM, 2013, pp. 562–567
   mine SO for code snippets that are clones to a snippet in the client system  

L. Ponzanelli, G. Bavota, M. D. Penta, R. Oliveto, and M. Lanza,
“Mining stackoverflow to turn the ide into a self-confident programming
prompter,” in Proceedings of the 10th IEEE Working Conference on
Mining Software Repositories (MSR), 2014. ACM, 2014, pp. 102–111
   mine SO for code snippets that are clones to a snippet in the client system  

L. Ponzanelli, A. Bacchelli, and M. Lanza, “Seahawk: Stack overflow in
the ide,” in 2013 35th International Conference on Software Engineering
(ICSE), May 2013, pp. 1295–1298
  tool to recommend SO snippets

% problems

zhang18icse 
  http://web.cs.ucla.edu/~tianyi.zhang/examplecheck.pdf
   Online
    31% contain
    potential API misuse that could produce symptoms such as program
    crashes, resource leaks, and incomplete actions


Felix Fischer, Konstantin Böttinger, Huang Xiao, Christian Stransky, Yasemin
Acar, Michael Backes, and Sascha Fahl. 2017. Stack Overflow Considered Harmful?
The Impact of Copy&Paste on Android Application Security. In Security and
Privacy (SP), 2017 IEEE Symposium on. IEEE, 121–136

  Fischer et al. investigate security-related
  code on Stack Overflow and find that 29% is insecure [9]. They
  further apply clone detection to check whether insecure code is
  reused from Stack Overflow to Android applications on Google
  Play and find that insecure code may have been copied to over
  1 million Android apps. 

Christoph Treude and Martin P Robillard. 2017. Understanding Stack Overflow
Code Fragments. In Proceedings of the 33rd International Conference on Software
Maintenance and Evolution. IEEE
   Treude and Robillard conduct a survey
  to investigate comprehension difficulty of code examples in Stack
  Overflow [29]. The responses from GitHub users indicate that less
  than half of the SO examples are self-explanatory






% Code flow.
Regex flow is a particular type of code flow.
Zhang \etal questioned whether Stack Overflow posts have API usage violations~\cite{Zhang2018AreSOCodeExamplesReliable}, and reported that Java code snippets containing regexes may not have correct exception handling.
Our characterization of behavioral false friendships is another factor for developers engaged in ``Stack Overflow-driven development'' to consider.
Code flow from Internet sources to source code has been studied from a security perspective in Java~\cite{Fischer2017SOHarmfulSecSnippets}.
Since SL regexes can lead to \REDOS vulnerabilities, the performance false friendships component of our work is in a similar vein.
Baltes and Diehl have reported that Stack Overflow snippets are often used without attribution in Java projects on GitHub~\cite{Baltes2019SOAttribution}.
Though our evidence is circumstantial (identical regexes can be independently derived), we XXX with them.

Abdalkareem \etal use code clone techniques to identify code snippets from Stack Overflow in Android applications~\cite{Abdelkareem2017SOCodeReuseInAndroid}.
In our case we are solely concerned about regexes, and could use exact string matching rather than code clone techniques.
However, these techniques would be helpful in future research on ``regex siblings''.

\JD{
Stack Overflow use across languages~\cite{Allamanis2013SOQuestions}.
Insights about the categories of programming tasks that are more common in various languages.
Reported overlap of question types between Python and Java, suggesting language independence of programming tasks.

False friendships could be detected using ``evil test strings''~\cite{Larson2016EvilTestStrings} and language-specific checking tools along the lines of ACRE~\cite{Larson2018AutomaticCheckingOfRegexes}.

The npm and PHP registries are duplicated on Cuba's SNET~\cite{Pujol2017CubanSNET}!
}





% portability?






% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------


% Empirical regex studies.
The empirical study of regex use is a recent endeavor, pioneered by Stolee.
Several lines of research have resulted.
Chapman and Stolee assessed the use of different regex features in Python~\cite{Chapman2016RegexUsageInPythonApps}.
Chapman, Wang, and Stolee assessed the understandability of functionally-equivalent regexes and determined community preferences based on the Chapman and Stolee's Python corpus~\cite{Chapman2017RegexComprehension}.
Wang and Stolee have reported that regexes appear to be relatively poorly tested in Java applications~\cite{Wang2018RegexTestCoverage}.
Davis \etal reported that SL regexes appear in 1-3\% of the modules in the \npm and \pypi registries.
Our polyglot regex corpus will permit the generalization of some of these results to other programming languages.
\JD{Paragraph comparing and contrasting our survey with the Chapman & Stolee survey? We already mentioned it in the background.}


% Code flow.
% Regex flow is a particular type of code flow.
% Zhang \etal questioned whether Stack Overflow posts have API usage violations~\cite{Zhang2018AreSOCodeExamplesReliable}, and reported that Java code snippets containing regexes may not have correct exception handling.
% Our characterization of behavioral false friendships is another factor for developers engaged in ``Stack Overflow-driven development'' to consider.
% Code flow from Internet sources to source code has been studied from a security perspective in Java~\cite{Fischer2017SOHarmfulSecSnippets}.
% Since SL regexes can lead to \REDOS vulnerabilities, the performance false friendships component of our work is in a similar vein.
% Baltes and Diehl have reported that Stack Overflow snippets are often used without attribution in Java projects on GitHub~\cite{Baltes2019SOAttribution}.
% Though our evidence is circumstantial (identical regexes can be independently derived), we XXX with them.

% Abdalkareem \etal use code clone techniques to identify code snippets from Stack Overflow in Android applications~\cite{Abdelkareem2017SOCodeReuseInAndroid}.
% In our case we are solely concerned about regexes, and could use exact string matching rather than code clone techniques.
% However, these techniques would be helpful in future research on ``regex siblings''.

% \JD{
% Stack Overflow use across languages~\cite{Allamanis2013SOQuestions}.
% Insights about the categories of programming tasks that are more common in various languages.
% Reported overlap of question types between Python and Java, suggesting language independence of programming tasks.

% False friendships could be detected using ``evil test strings''~\cite{Larson2016EvilTestStrings} and language-specific checking tools along the lines of ACRE~\cite{Larson2018AutomaticCheckingOfRegexes}.

% The npm and PHP registries are duplicated on Cuba's SNET~\cite{Pujol2017CubanSNET}!
% }






\DY{
Software reuse can significantly improve software quality and productivity.
-- Frakes et al.~\cite{Frakes1991} 1991;
-- Krueger~\cite{Krueger:1992:SR:130844.130856} 1992;
-- Lim~\cite{Lim:1994:ERQ:624603.625375} 1994;
-- Mohagheghi and Conradi~\cite{Mohagheghi:2007:QPE:1290895.1290919} 2007;
-- Spoelstra et al.~\cite{Spoelstra:2011:SRA:1982185.1982255} 2011

Empirical study to support practitioners in executing reuse tasks
-- Mili et al.~\cite{Mili1995} 1995;
-- Frakes and Kang~\cite{Frakes2005} 2005;

Reuse in practice (empirical study)
-- Frakes and Fox, 1996; 
-- Rine, 1997; 
-- Hallsteinsen and Paci, 1997; 
-- Morisio et al., 2002a; 
-- Mohagheghi and Conradi, 2007; 
-- Land et al., 2009; 
-- Heinemann et al., 2011; 
-- Dubinsky et al., 2013; 
-- Stol et al., 2014

the opportunities, challenges, and risks of employing thirdparty reusables have been studied  
-- Bauer et al., 2012; 
-- Raemaekers et al., 2012a; 2012b; 
-- Businge et al., 2012; 
-- Mileva et al., 2010

for a large number of software producing companies, finding, adopting, and sustaining an adequate reuse strategy remains a challenge 
-- Morisio et al., 2002a; 
-- Marcus et al, 2003; 
-- Bauer, 2015

the means to effect reuse are often limited due to lack of tool support or organizational limitations
-- Dubinsky et al., 2013


Frakes and Fox~\cite{Frakes1996} -- improving a parts-based reuse process using a model of the ways the reuse process can fail. Successful reuse depends on the satisfaction of seven main conditions. Figure 1: 1.Try to Reuse -> 2.Part Exists -> 3.Part Available -> 4. Part Found -> 5. Part Understood -> 6. Part Valid -> 7. Part Integratable.

Bauera and Vetro~\cite{BAUER2016545} 2016 -- empirical study on software reuse at two large software-producing companies. Both companies perform pragmatic reuse of code produced within the company, not leveraging other available artefacts. In both cases, a lack of reuse led to duplicate implementations.

Code Reuse in Open Source Software
Stefan Haefliger, Georg von Krogh, Sebastian Spaeth 2008

}

